CLIP-RT: Learning Language-Conditioned Robotic Policies from Natural Language Supervision

Teaching robots desired skills in real-world environments remains challenging, especially for non-experts. A key bottleneck is that collecting robotic data often requires expertise or specialized hardware, limiting accessibility and scalability. We posit that natural language offers an intuitive and accessible interface for robot learning. To this end, we study two aspects: (1) enabling non-experts to collect robotic data through natural language supervision (e.g., "move the arm to the right") and (2) training robot policies directly from this supervision. Specifically, we introduce a data collection framework that collects robot demonstrations based on natural language supervision and further augments these demonstrations. We then present CLIP-RT, a new vision-language-action (VLA) model that learns language-conditioned visuomotor policies from this supervision. CLIP-RT adapts the pretrained CLIP model and learns to predict language-based motion primitives via contrastive imitation learning. We train CLIP-RT on the Open X-Embodiment dataset and finetune it on in-domain data collected by our framework. In real-world evaluations, CLIP-RT demonstrates strong capabilities in learning novel manipulation skills, outperforming OpenVLA (7B parameters) by 24% in average success rates, while using 7x fewer parameters (1B). We further assess CLIP-RT's capabilities in few-shot generalization and collaborative scenarios involving large pretrained models or humans. In simulated environments, CLIP-RT also yields strong performance, achieving a 93.1% average success rate on the LIBERO benchmark with an inference throughput of 163 Hz.

==> sections/04.1_exp_main.tex <==
\subsection{Comparison with State-of-the-Art (OpenVLA)}
\label{ssec:comparison_openvla}


Figure~\ref{fig:result_performance} compares the success rates of CLIP-RT and OpenVLA on \emph{Common} and \emph{Novel} tasks. In the Common tasks, which are closely aligned with the pretraining data, both models perform well, with CLIP-RT achieving a success rate 54\% and OpenVLA trailing slightly at 51\%. However, the performance gap becomes more pronounced in the Novel tasks, where CLIP-RT reaches 53\% on average, notably surpassing OpenVLA’s 29\%. These findings suggest that while OpenVLA and CLIP-RT handle familiar tasks similarly, CLIP-RT generalizes more effectively to tasks that deviate from the pretraining distribution (Open-X Embodiment dataset).

To investigate the source of this improved generalization, we conducted both single-task and multi-task training on the Novel tasks (see \ref{fig:single}). In \emph{single-task training}, each model was trained only on one Novel task at a time. In \emph{multi-task training}, on the contrary, each model learned all nine Novel tasks simultaneously. In all tasks, CLIP-RT exhibited more substantial gains in multi-task training than in single-task training, with an average improvement 13\% compared to OpenVLA’s 7\%. These results highlight CLIP-RT's ability to leverage knowledge transfer across tasks, which is particularly beneficial when training examples are scarce.

We further explored the capacity of both models to learn from minimal demonstrations by measuring success rates under 1-, 5-, and 10-shot training regimes (see Figure~\ref{fig:fewshot}).
We selected three Novel tasks where both models performed relatively well on average.
In all configurations, CLIP-RT consistently outperformed OpenVLA, indicating superior few-shot learning. 
Such adaptability is particularly critical for robotics, where pretraining data~\cite{padalkar2023open} cannot encompass every possible task, necessitating models that can rapidly acquire novel skills (Novel tasks) from minimal demonstrations.

We delve deeper into how language-based action representations drive CLIP-RT’s advantages in Section~\ref{ssec:ablation_study}, and provide additional comparative analyses of CLIP-RT and OpenVLA in Appendix~\ref{ssec:additional_analysis}.  




\subsection{Ablation Study}
\label{ssec:ablation_study}
We conduct an ablation study to examine the roles of CLIP-RT’s key components by comparing three variants—\emph{CLIP-RT-Action}, \emph{CLIP-RT-Passive}, and \emph{CLIP-RT-Zero}. Their performance is summarized in Figure~\ref{fig:result_performance}.


\noindent \textbf{Effect of Representing Actions in Natural Language.}
The results reveal that \textit{CLIP-RT-Action}, which learns action tokens from scratch, generally lags behind \textit{CLIP-RT}. 
We hypothesize that \textbf{CLIP-RT} benefits from the pretrained vision-language representations in CLIP~\cite{radford2021learning}, allowing it to align actions with semantic concepts more effectively.
In particular, CLIP’s language embeddings offer a well-structured space for representing actions, which should facilitate more consistent and meaningful action reasoning.
To verify this, Figure~\ref{fig:umanp} shows the embeddings of 58 language-based actions. 
We can see that CLIP-RT naturally groups related actions and encodes their compositional structures more effectively than CLIP-RT-Action, where each action token is learned independently. 
Closely related actions (\textit{e.g.,} “move left a lot” and “move left”) appear nearer in the embedding space, providing a stable foundation for CLIP-RT to reason about actions.

%Moreover, \textit{CLIP-RT-Action} notably underperforms \textit{CLIP-RT} in tasks that require precise movements, such as \emph{Erase the Whiteboard}, \emph{Open the Trashcan}, and \emph{Stamp}. 
%We hypothesize that CLIP-RT’s advantage arises from its natural language representation, which offers richer semantic context and compositionality. 
%For example, once CLIP-RT learns that “\emph{move forward a little}” denotes fine control when the end-effector is close to a target object, it can reuse this insight across contexts that require subtle movements by sharing tokens like “move left \emph{a little}” and “lower arm \emph{a little}”. 
%In contrast, CLIP-RT-Action treats each token as independent, making it more difficult to transfer knowledge between actions.



\noindent \textbf{Impact of Stochastic Trajectory Diversification.}
CLIP-RT-Passive, which omits Stochastic Trajectory Diversification (STD), struggles in most tasks, highlighting the critical role of STD in model performance. 
STD enables the model to learn from diverse possible trajectories, enhancing its robustness and generalization capabilities. 
By exploring deviations from optimal trajectories, the model becomes adept at recovering from nonoptimal states and adapting to unexpected variations in the robot's position. 
Detailed qualitative examples that illustrate the role of STD in recovery are provided in the Appendix~\ref{ssec:qualitative_std}. 


\noindent \textbf{Importance of In-Domain Data.}
Finally, CLIP-RT-Zero is trained solely on the Open X-Embodiment dataset, without utilizing any in-domain data from our Common or Novel tasks. Its weak performance underscores the necessity of domain-specific fine-tuning. 
Although large-scale pretrained models offer strong initialization, adaptation to new environments remains crucial to achieving higher success rates. 
Although this adaptation requires additional data collection, our framework is designed to make collecting in-domain data more intuitive, thus enabling fine-tuning in practice. 



==> sections/04.2_few_shot.tex <==

\subsection{Few-shot Experiments}
Few-shot experiments assess the generalization ability of CLIP-RT, CLIP-RT-Action, and OpenVLA with limited training data. Figure~\ref{fig:fewshot} presents the success rates across different numbers of trajectories (\textit{i.e.}, 1, 5, and 10-shot settings). CLIP-RT consistently outperforms both baselines, demonstrating strong adaptability to novel tasks. While CLIP-RT-Action achieves competitive performance in the early stages (1-5 shots), CLIP-RT surpasses it as training progresses. OpenVLA struggles to generalize effectively, exhibiting the lowest success rates across all shot levels. Notably, the largest performance improvement is observed from 1-shot to 5-shot, indicating that CLIP-RT rapidly benefits from additional trajectories.


A task-wise breakdown reveals that CLIP-RT maintains a consistent advantage over OpenVLA and CLIP-RT-Action in most tasks. In "Open the Cabinet," both CLIP-RT and CLIP-RT-Action perform similarly, while OpenVLA remains significantly lower. In "Erase the Whiteboard," CLIP-RT achieves the highest success rate, whereas the gap between CLIP-RT-Action and OpenVLA remains small. Interestingly, in "Close the Laptop," CLIP-RT-Action initially outperforms CLIP-RT, but as training progresses, CLIP-RT eventually matches its performance. This suggests that CLIP-RT-Action benefits from structured action representation in early-stage learning but lacks the robustness of CLIP-RT in long-term adaptation.

==> sections/99_guidelines.tex <==
\section{Introduction}
This demo file is intended to serve as a ``starter file" for the
Robotics: Science and Systems conference papers produced under \LaTeX\
using IEEEtran.cls version 1.7a and later.  

\section{Section}

Section text here. 

\subsection{Subsection Heading Here}
Subsection text here.

\subsubsection{Subsubsection Heading Here}
Subsubsection text here.


\section{RSS citations}

Please make sure to include \verb!natbib.sty! and to use the
\verb!plainnat.bst! bibliography style. \verb!natbib! provides additional
citation commands, most usefully \verb!\citet!. For example, rather than the
awkward construction 

{\small
\begin{verbatim}
\cite{kalman1960new} demonstrated...
\end{verbatim}
}

\noindent
rendered as ``\cite{kalman1960new} demonstrated...,''
or the
inconvenient 

{\small
\begin{verbatim}
Kalman \cite{kalman1960new} 
demonstrated...
\end{verbatim}
}

\noindent
rendered as 
``Kalman \cite{kalman1960new} demonstrated...'', 
one can
write 

{\small
\begin{verbatim}
\citet{kalman1960new} demonstrated... 
\end{verbatim}
}
\noindent
which renders as ``\citet{kalman1960new} demonstrated...'' and is 
both easy to write and much easier to read.
  
\subsection{RSS Hyperlinks}

This year, we would like to use the ability of PDF viewers to interpret
hyperlinks, specifically to allow each reference in the bibliography to be a
link to an online version of the reference. 
As an example, if you were to cite ``Passive Dynamic Walking''
\cite{McGeer01041990}, the entry in the bibtex would read:

{\small
\begin{verbatim}
@article{McGeer01041990,
  author = {McGeer, Tad}, 
  title = {\href{http://ijr.sagepub.com/content/9/2/62.abstract}{Passive Dynamic Walking}}, 
  volume = {9}, 
  number = {2}, 
  pages = {62-82}, 
  year = {1990}, 
  doi = {10.1177/027836499000900206}, 
  URL = {http://ijr.sagepub.com/content/9/2/62.abstract}, 
  eprint = {http://ijr.sagepub.com/content/9/2/62.full.pdf+html}, 
  journal = {The International Journal of Robotics Research}
}
\end{verbatim}
}
\noindent
and the entry in the compiled PDF would look like:

\def\tmplabel#1{[#1]}

\begin{enumerate}
\item[\tmplabel{1}] Tad McGeer. \href{http://ijr.sagepub.com/content/9/2/62.abstract}{Passive Dynamic
Walking}. {\em The International Journal of Robotics Research}, 9(2):62--82,
1990.
\end{enumerate}
%
where the title of the article is a link that takes you to the article on IJRR's website. 


Linking cited articles will not always be possible, especially for
older articles. There are also often several versions of papers
online: authors are free to decide what to use as the link destination
yet we strongly encourage to link to archival or publisher sites
(such as IEEE Xplore or Sage Journals).  We encourage all authors to use this feature to
the extent possible.

\section{Conclusion} 
\label{sec:conclusion}

The conclusion goes here.

\section*{Acknowledgments}

%% Use plainnat to work nicely with natbib. 
